Temporal-Difference Learning Using Distributed Error Signals

A computational problem in biological reward-based learning is how credit assignment is performed in the nucleus accumbens (NAc). Much research suggests that NAc dopamine encodes temporal-difference (TD) errors for learning value predictions. However, dopamine is synchronously distributed in regionally homogeneous concentrations, which does not support explicit credit assignment (like used by backpropagation). It is unclear whether distributed errors alone are sufficient for synapses to make coordinated updates to learn complex, nonlinear reward-based learning tasks. We design a new deep Q-learning algorithm, Artificial Dopamine, to computationally demonstrate that synchronously distributed, per-layer TD errors may be sufficient to learn surprisingly complex RL tasks. We empirically evaluate our algorithm on MinAtar, the DeepMind Control Suite, and classic control tasks, and show it often achieves comparable performance to deep RL algorithms that use backpropagation.

==> conclusion.tex <==
\section{Conclusion}

We proposed \name, a deep Q-learning algorithm and architecture that alleviates several contradictions between deep RL and biological learning, particularly due to the biological implausibility of backpropagation.
Each Local-Forward cell computes its own local TD error, based on the difference between its prediction and the TD target.
The TD target is provided to all cells; in parts of the brain this could be achieved by a global signal via dopamine neurons.
To send information to lower layers, upper layers send their activations forward in time to the layer below, hence the name Local-Forward.
We empirically showed that Local-Forward can learn control tasks in the MinAtar environments, and even surpasses a similar-sized DQN in performance in 2 environments.
Thus, we believe it warrants further investigation.
We outline some areas for investigating potential improvements in our limitations.

